Reducing Runtime Overhead via Use-Based Migration in Neutral Atom Quantum Architectures

Neutral atoms are a promising choice for scalable quantum computing architectures. Features such as long distance interactions and native multiqubit gates offer reductions in communication costs and operation count. However, the trapped atoms used as qubits can be lost over the course of computation and due to adverse environmental factors. The value of a lost computation qubit cannot be recovered and requires the reloading of the array and rerunning of the computation, greatly increasing the number of runs of a circuit. Software mitigation strategies exist but exhaust the original mapped locations of the circuit slowly and create more spread out clusters of qubits across the architecture decreasing the probability of success. We increase flexibility by developing strategies that find all reachable qubits, rather only adjacent hardware qubits. Second, we divide the architecture into separate sections, and run the circuit in each section, free of lost atoms. Provided the architecture is large enough, this resets the circuit without having to reload the entire architecture. This increases the number of effective shots before reloading by a factor of two for a circuit that utilizes 30% of the architecture. We also explore using these sections to parallelize execution of circuits, reducing the overall runtime by a total 50% for 30 qubit circuit. These techniques contribute to a dynamic new set of strategies to combat the detrimental effects of lost computational space.

==> figs/basic-circuit.tex <==
\Qcircuit @R=0.25em @C=0.75em @!R{
\lstick{q_0} & \gate{X} & \qw & \ctrl{1} & \qw & \ctrl{1} & \qw \\
\lstick{q_1} & \qw & \qw & \targ & \qw & \ctrl{1} & \qw \\
\lstick{q_2} & \qw & \qw & \qw & \qw & \targ & \qw
}

==> figs/hole-fidelity-cnu-30.tex <==
% This file was automatically generated by python latextools.
% https://github.com/cduck/latextools
%
% \usepackage{tikz}
% \usepackage{pgfplots}
%
% % Setup package: tikz
% \usetikzlibrary{patterns}
% \usetikzlibrary{arrows}
% \usetikzlibrary{external}
%
% % Setup package: pgfplots
% \pgfplotsset{{compat=1.14}}
%
% Pgfplots figure
\begin{tikzpicture}[baseline,scale=1,trim axis left,trim axis right]
%\pgfplotsset{every axis/.append style={thick}}
\pgfplotsset{every tick label/.append style={font=\small}}
\pgfplotsset{every axis label/.append style={font=\small}}

    \begin{axis}[
        name=plot11,
        title={Shot Success Rate Drop (CNU, 30 qubits)},
        xlabel={Number of Holes},
        ylabel={Estimated Shot Success},
        width={\columnwidth},
        height={0.8*\columnwidth},
    %    restrict x to domain=0:0,
    %    xtick distance=25,
        xmin=0, ymin=0, ymax=0.831983661149046,
        ,
        legend style={
            draw=none,
            at={(0.5,1)},
            anchor=north,
    %        fill=none,
            font=\small},
    %    legend columns=-1,
        ,
        clip=false,
        axis line style={draw=none},
        tick style={draw=none},,
        legend columns=6, legend cell align={left}, legend style={at={(1.3,1.05)},anchor=north}, mark size=3pt,
    ]
        \addplot[color=white, ]
            table[x=number-of-holes 0, y=c-smallreroute----mid estimated-shot-success 0, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{c. small+reroute   , MID:~~};

        \addplot[color={rgb,405:red,0;green,205;blue,110}, thick, mark=x, ]
            table[x=number-of-holes 1, y=3 estimated-shot-success 1, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{3~~};

        \addplot[color={rgb,405:red,125;green,0;blue,255}, thick, mark=x, ]
            table[x=number-of-holes 2, y=5 estimated-shot-success 2, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{5~~};

        \addplot[color=white, ]
            table[x=number-of-holes 3, y=wear-leveling--mid estimated-shot-success 3, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{wear-leveling , MID:~~};

        \addplot[color={rgb,405:red,0;green,205;blue,110}, thick, mark=+, ]
            table[x=number-of-holes 4, y=3 estimated-shot-success 4, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{3~~};

        \addplot[color={rgb,405:red,125;green,0;blue,255}, thick, mark=+, ]
            table[x=number-of-holes 5, y=5 estimated-shot-success 5, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{5~~};

        \addplot[color=white, ]
            table[x=number-of-holes 6, y=wear-leveling-constrained-mid estimated-shot-success 6, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{wear-leveling constrained, MID:~~};

        \addplot[color={rgb,405:red,0;green,205;blue,110}, thick, mark=o, mark size=2pt, ]
            table[x=number-of-holes 7, y=3 estimated-shot-success 7, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{3~~};

        \addplot[color={rgb,405:red,125;green,0;blue,255}, thick, mark=o, mark size=2pt, ]
            table[x=number-of-holes 8, y=5 estimated-shot-success 8, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{5~~};

        \addplot[color=white, ]
            table[x=number-of-holes 9, y=c-smallim-reroute---mid estimated-shot-success 9, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{c. small+im reroute  , MID:~~};

        \addplot[color={rgb,405:red,0;green,205;blue,110}, thick, mark=square, ]
            table[x=number-of-holes 10, y=3 estimated-shot-success 10, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{3~~};

        \addplot[color={rgb,405:red,125;green,0;blue,255}, thick, mark=square, ]
            table[x=number-of-holes 11, y=5 estimated-shot-success 11, col sep=comma]
            {data/hole-fidelity-cnu-shot-success-rate-drop-cnu-30-qubits.csv}
        ;%node [anchor=north east] {...};
        \addlegendentry{5~~};


    %
    \end{axis}

\end{tikzpicture}


==> figs/hole-fidelity-cuccaro-30.tex <==
% This file was automatically generated by python latextools.
% https://github.com/cduck/latextools
%
% \usepackage{tikz}
% \usepackage{pgfplots}
%
% % Setup package: tikz
% \usetikzlibrary{patterns}
% \usetikzlibrary{arrows}
% \usetikzlibrary{external}
%
% % Setup package: pgfplots
% \pgfplotsset{{compat=1.14}}
%
% Pgfplots figure
\begin{tikzpicture}[baseline,scale=1,trim axis left,trim axis right]
%\pgfplotsset{every axis/.append style={thick}}
\pgfplotsset{every tick label/.append style={font=\small}}
\pgfplotsset{every axis label/.append style={font=\small}}

    \begin{axis}[
        name=plot11,
        title={Shot Success Rate Drop (Cuccaro, 30 qubits)},
        xlabel={Number of Holes},
        ylabel={},
        width={\columnwidth},
        height={0.8*\columnwidth},
    %    restrict x to domain=0:0,
    %    xtick distance=25,
        xmin=0, ymin=0, ymax=0.7002145441499361,
        ,
        legend style={
            draw=none,
            at={(0.5,1)},
            anchor=north,
    %        fill=none,
            font=\small},
    %    legend columns=-1,
        ,
        clip=false,
        axis line style={draw=none},
        tick style={draw=none},,
        legend columns=6, legend cell align={left}, legend style={at={(1.3,1.05)},anchor=north}, mark size=3pt,
    ]
        \addplot[color=white, ]
            table[x=number-of-holes 0, y=0, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color={rgb,405:red,0;green,205;blue,110}, thick, mark=x, ]
            table[x=number-of-holes 1, y=1, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color={rgb,405:red,125;green,0;blue,255}, thick, mark=x, ]
            table[x=number-of-holes 2, y=2, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color=white, ]
            table[x=number-of-holes 3, y=3, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color={rgb,405:red,0;green,205;blue,110}, thick, mark=+, ]
            table[x=number-of-holes 4, y=4, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color={rgb,405:red,125;green,0;blue,255}, thick, mark=+, ]
            table[x=number-of-holes 5, y=5, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color=white, ]
            table[x=number-of-holes 6, y=6, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color={rgb,405:red,0;green,205;blue,110}, thick, mark=o, mark size=2pt, ]
            table[x=number-of-holes 7, y=7, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color={rgb,405:red,125;green,0;blue,255}, thick, mark=o, mark size=2pt, ]
            table[x=number-of-holes 8, y=8, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color=white, ]
            table[x=number-of-holes 9, y=9, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color={rgb,405:red,0;green,205;blue,110}, thick, mark=square, ]
            table[x=number-of-holes 10, y=10, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};

        \addplot[color={rgb,405:red,125;green,0;blue,255}, thick, mark=square, ]
            table[x=number-of-holes 11, y=11, col sep=comma]
            {data/hole-fidelity-cuccaro-shot-success-rate-drop-cuccaro-30-qubits.csv}
        ;%node [anchor=north east] {...};


    %
    \end{axis}

\end{tikzpicture}


==> text/acknowledgements.tex <==
\newcommand\acksname{Acknowledgments}
\specialcomment{acks}{%
  \begingroup
  \section*{\acksname}
  \phantomsection\addcontentsline{toc}{section}{\acksname}
}

\begin{acks}

Thank you to Max Siefert, Jason Chadwick and Natalia Nottingham for their helpful conversations in developing this work.
\end{acks}
